Planning Strategies for Lane Reversals in Transportation Networks

This paper studies strategies to optimize the lane configuration of a transportation network for a given set of Origin-Destination demands using a planning macroscopic network flow model. The lane reversal problem is, in general, NP-hard since the optimization is made over integer variables. To overcome this burden, we reformulate the problem using a piecewise affine approximation of the travel latency function which allows us to exploit the total unimodularity property of Integer Linear Programming (ILP). Consequently, we transform the ILP problem to a linear program by relaxing the integer variables. In addition, our method is capable of solving the problem for a desired number of lane reversals which serves to perform cost-benefit analysis. We perform a case study using the transportation network of Eastern Massachusetts (EMA) and we test our method against the original lane configuration and a projected lower bound solution. Our empirical results quantify the travel time savings for different levels of demand intensity. We observe reduction in travel times up to 40% for certain links in the network.

==> tables/table.tex <==
\begin{tabular}{|l|llll|}
\hline
\textbf{Policy} & \textbf{AM} & \textbf{MD} & \textbf{PM} & \textbf{NT} \\
\hline 

\hline
$\mathcal{P}_{ij}$                            &   -29.83 &    -8.77 &    -6.64 &   -26.00 \\
$\mathcal{R}_{ij}$                            &   -33.33 &   -28.74 &   -29.20 &   -40.67 \\
$\mathcal{R}_{ij}\rightarrow\mathcal{P}_{ij}$ &   -13.72 &    -9.38 &   -10.89 &   -15.75 \\
$\mathcal{P}_{i}+\mathcal{R}_{ij}$            &       -5.3 &       -5.3 &       -5.1 &         -7.0 \\
\hline

\hline
\end{tabular}

==> tables/table2.tex <==
\begin{tabular}{|l|llll|}
\hline

 & \textbf{AM} & \textbf{MD} & \textbf{PM} & \textbf{NT} \\
\hline

\hline
%$\mu_{\bu}$                                   &   2.38 &   2.34 &    2.35 &   2.32 \\
%$\sigma_\bu$                                  &  0.29 &  0.26 &  0.29 &  0.34 \\



%\hline
$\bar{\zeta}_0$                            &   57.03 &   16.62 &   34.77 &    17.64 \\
%$\sigma_{\blambda^0}$                         &    112.25 &     62.79 &     91.15 &     44.76 \\


%\hline
$\bar{\zeta}_{\bu^*}$                     &   20.44 &   4.10 &   6.80 &   6.24 \\
%$\sigma_{\blambda_i(\bu^*)}$                  &     44.16 &     22.39 &     29.61 &     17.25 \\

%\hline
$\bar{\zeta}_{\br^*}$                      &     36.71 &     13.23 &     28.36 &     11.49 \\
%$\sigma_{\blambda^0+\br^*}$                   &   69.46 &   42.87 &   64.49 &   28.07 \\

\hline

\hline

\end{tabular}

